An efficient approach for nonconvex semidefinite optimization via customized alternating direction method of multipliers

We investigate a class of general combinatorial graph problems, including MAX-CUT and community detection, reformulated as quadratic objectives over nonconvex constraints and solved via the alternating direction method of multipliers (ADMM). We propose two reformulations: one using vector variables and a binary constraint, and the other further reformulating the Burer-Monteiro form for simpler subproblems. Despite the nonconvex constraint, we prove the ADMM iterates converge to a stationary point in both formulations, under mild assumptions. Additionally, recent work suggests that in this latter form, when the matrix factors are wide enough, local optimum with high probability is also the global optimum. To demonstrate the scalability of our algorithm, we include results for MAX-CUT, community detection, and image segmentation benchmark and simulated examples.

==> convergence.tex <==

\section{Convergence analysis}





%In this section, we aim to establish the global convergence of Algorithms 1 to a stationary point of \eqref{eq:FormulationXxy1} under some conditions~.



\begin{Assumption}
\begin{enumerate}
\item
The sequences $\{f(Z^k)\}$ and $\{\Lambda_1^k,\Lambda_2^k\}$ are bounded in norm.
\item
$f(Z)$ has bounded non-convexity. Mathematically, for any $Z_1,Z_2\in\symm^n$, it holds that $f(Z_1) \ge f(Z_2) + \langle \nabla f(Z_2), Z_1-Z_2\rangle - \frac{L_f}{2}\|Z_1-Z_2\|_F^2$ with $L_f < +\infty$.
\end{enumerate}
\end{Assumption}


\begin{thm}\label{lemma:LagDecentXxy}
If Assumption \ref{Assumption:BoundedDualXxy} holds, and given a sequence $\{\rho^k\}$ such that
\[
\rho^k\left(1- \frac{\sqrt{\lambda_N^2+4\lambda_N}-\lambda_N}{2}\right) > L_f, \sum\frac{\rho^{k+1}}{(\rho^k)^2} < \infty, \text{ and } \sum\frac{1}{\rho^k} < \infty,
\]
with $\lambda_N = \|Y^{k+1}\|^2_2$, then
 $\{Z^k, X^k, Y^k\}$ generated by Algorithm  \ref{a:matrix} will globally converge to a stationary point of (\ref{eq:FormulationXxy1}).
\end{thm}
\begin{proof}
  See section \ref{sec:matrixproof} in the appendix.
\end{proof}

%If we pick $r = 1$, then $X$ and $Y$ are length-$n$ binary vectors, and $x = X$ is a locally optimal solution of \eqref{eq:main}. If $\frac{r(r+1)}{2} > n$ (e.g, $\ceil{\sqrt{2n}}$), $X$ can be projected on a rank-1 solution using a randomization technique popularized by Goemans/Williamson (\cite{goemans1995improved}). For max-cut problem, such randomization technique can generate an approximately optimal cut within a ratio of $0.878$.


\begin{cor}
	If $r \geq \ceil{\sqrt{2n}}$ and the  stationary point of Algorithm \ref{a:matrix} converges to a second order critical point of \eqref{eq:FormulationXxy1}, then it is globally optimal for the convex relaxation of \eqref{eq:FormulationXxy0SymFact}~\cite{boumal2016non}.
\end{cor}
%\begin{proof}
%  Given the search space of the SDR \eqref{eq:FormulationXxy0SDR} is compact and that of \eqref{eq:FormulationXxy1} is a smooth manifold, combining Theorem \ref{lemma:LagDecentXxy} and Theorem 2 in~\cite{boumal2016non} will trivially result to the conclusion.
%\end{proof}

Unfortunately, the extension of KKT stationary points to global minima is not yet known when $\frac{r(r+1)}{2} < n$ (\ie, $r = 1$). However, our empirical results suggest that even when $r = 1$, often a local solution to \eqref{eq:FormulationXxy1} well-approximates the global solution to \eqref{eq:main}.


%\section{BINARY VECTOR FORM}
\paragraph{VECTOR FORM}
We begin by considering a simple reformulation of \eqref{eq:main} using only vector variables
%. To solve it directly in the ADMM framework, we first reformulate it in the following via introducing an auxiliary variable $y$
\begin{equation}
\label{eq:Formulation3}
\begin{array}{ll}
\minimize{x,y\in \reals^n}& x^TCx \\
\st& y \in \{-1,1\}^n\nonumber\\
    & x = y.\nonumber
    \end{array}
\end{equation}
This is similar to the nonconvex formulations proposed in \cite{boyd2011distributed}, Chapter 9.1.




\begin{definition}\label{def:L}
$x^TCx$ is $L_1-$smooth function, that is, any $x_1, x_2$, $\| 2Cx_1 - 2Cx_2\| \le L_1\|x_1 - x_2\|$.\\
\end{definition}



\begin{definition}\label{Definition:L_H}
$L_H\in\reals_{+}$ is the smallest number such that $-L_HI \preceq 2C$, where $2C$ is the Hessian of the objective function of \eqref{eq:main}. In other words, the Hessian is lower bounded.
\end{definition}

\begin{Assumption}\label{Assumption:Df}
%\eqref{eq:main} is bounded, i.e.,
The value $x^TCx$ is lower bounded over $x\in \{-1,1\}^n$.
\end{Assumption}




\begin{thm}\label{lemma:LagDecent}
%With the parameters $L_H$ and $L_1$ in Definition \ref{Definition:L_H} and \ref{def:L}, respectively,
Given the sequence $\{\rho^k\}$ such that
\[
(\rho^k)^2-L_H\rho^k - (\alpha+1)L_1^2 > 0,\rho^k > L_H, \alpha > 0
\]
under Algorithm \ref{a:vector} the augmented Lagrangian monotonically decreases
\[
\mathcal{L}(y^{k+1},x^{k+1};\mu^{k+1}) - \mathcal{L}(y^{k},x^{k};\mu^{k}) \le - c_1^k\|x^{k+1} - x^{k}\|_F^2
\]
with $c_1^k = \frac{\rho^k-L_H}{2} - \frac{(\alpha+1)L_1^2}{2\rho^{k}} >0$.
With Assumption \ref{Assumption:Df} and $\rho^k > L_1$, the augmented Lagrangian  $\mL({y}^{k},{x}^k;{\mu}^k)$ is lower bounded and convergent.
Therefore, $\{{y}^k,{x}^k,{\mu}^k\}$ converge to $\{{y}^*,{x}^*,{\mu}^*\}$ a KKT solution of \eqref{eq:Formulation3} and
%$\lim_{k\to\infty}\{{y}^k,{x}^k,{\mu}^k\} = \{{y}^*,{x}^*,{\mu}^*\}$ and
${x}^* = {y}^*$.
\end{thm}
\begin{proof}
See section \ref{sec:vectorconvergence} in the appendix.
\end{proof}

\textit{Remark}: Convergence is also guaranteed under a constant penalty coefficient $\rho_k \equiv \rho^0$ ($\alpha=1$) satisfying $(\rho^0)^2-L_H\rho^0 - 2L_1^2 > 0$.
% can also guarantee the convergence. I
However, in implementation, we find empirically that increasing $\{\rho^k\}$ from a relatively small $\rho^0$  can encourage convergence to more useful global minima.
% to obtain a better numerical performance given the algorithm can be more sensitive to the initial with a large $\rho$.



\begin{cor}\label{thm:Convergence}
With the prerequisites in Theorem \ref{lemma:LagDecent} satisfied and $(y^*,x^*;\mu^*)$ as the accumulation point, we have that\\
\begin{enumerate}
	\item[i.]$\mu_i^*x_i^* \ge -\rho^*$ with $x^*\in\{-1,1\}^n$.
	\item[ii.] ${x}^*$ is a stationary point of the optimization problem $\min_{{x}}x^TCx+({\mu}^*)^T{x}$.
\end{enumerate}
 In particular for a convex function objective $f(x) = x^TCx$ ($C \succeq 0$), ${\mu}^* = 0$ indicates that the constraint $x\in\{-1,1\}^n$ is automatically satisfied; that is, the minimizer of $f(x)$ is the exact minimizer of \eqref{eq:main}.

% (\ref{eq:Formulation1}) could ignore the bivalent constraint. That is $\min_{x}f({x})$ has an optimum ${x}^*$ which satisfies $x\in\{-1,1\}^n$. In other words,

% the convex relaxation is \textit{exact}.
\end{cor}

\begin{proof}
See section \ref{sec:vectorconvergence} in the appendix.
\end{proof}





==> extra.tex <==




\section{Related works on ADMM}






In particular, it addresses a difficulty with the approach presented in \cite{burer2003nonlinear}, in which subproblems involve a quartic of the low-rank matrix variable $X$, and thus require iterative algorithms to solve the subproblems. \cite{burer2003nonlinear} uses an alternating linearization approach, but in fact this problem will arise for many other approaches, including ADMM or gradient descent. We address this issue by using a nonsymmetric parametrization: $Z = XY^T$ and $X = Y$; now, every subproblem involves only quadratics of the matrix variables, and can be solved directly.



Our main contribution is to prove the convergence of ADMM over this nonconvex problem to a KKT stationary point.
\footnote{In fact, our convergence can be generalized for any bounded Lipschitz continuous objective function $f(Z)$; we restrict to $f(Z)$ to ensure the subproblems are computationally cheap.}
In general,  convergence guarantees of ADMM over nonconvex problems are extremely limited, and are largely limited to cases where the nonconvexity is in the objective (e.g. with a simple nonconvex norm) \cite{hong2016convergence,wang2015global,li2015global,magnusson2016convergence, lu2017nonconvex,xu2012alternating}.
\red{The difficulty of dealing with nonconvexity in the constraint is...}
Finally, we point out that in cases where it is known that all stationary points are global optima (in particular [Pataki result]) our convergence proof thus shows convergence to a global solution.


\subsection{Notation}
We define $\mb 1$ as the vector of all 1's. We define $\symm^n$ and $\symm_+^n$ to be the set of symmetric and symmetric positive semidefinite (PSD) matrices of order $n$.

\section{move me elsewhere}
Our approach is extremely straightforward: we solve problem \eqref{eq:main} by introducing a dummy variable $Y$, and transforming the quadratic constraint $Z = XX^T$ to a bilinear one $Z = XY^T, \; X = Y$. We then solve this reformulated problem using ADMM, with two-variable splitting over the variable groups $Z,X$ and $Y$. Minimizing over $Z,X$ jointly results in solving a linear system of form
\[
\mathcal A(\mathcal A^*(\nu)) (G) + E = f
\]
where $G$ is positive definite, and is easy if inverting the operation $\mathcal A\mathcal A^*$ can be done easily. This covers all instances where $\mA$ is simple (e.g. $\mA = \diag(A)$  in combinatorial applications), or when $\mA$ is a structured operator (e.g.  discrete Fourier transform in phase retrieval).
Minimizing over $Y$ is a generalized projection problem, and is the solution to
\[
\min_{Y\in\mC} \langle Y - U, Y - U\rangle_H
\]
over some positive definite matrix $H$. For combinatorial problems, where $r = 1$, $H$ is diagonal, and the operation can be done in one step if $\mC$ is simple. Otherwise, simple iterative methods (such as projected gradient descent) can be used.


\paragraph{asdf}

The third category of approaches  often work very well for  specific applications, but are not always generalizable to larger classes of nonconvex problems.

A key issue with the convexified SDP is the resulting scalability, since in general solving large-scale SDPs with dense unstructured intermediate iterates is computationally complex and memory inefficient. In such cases, naive interior point or first order implementations cannot possibly scale well, requiring large matrix solves and eigenvalue decompositions at each iteration. By exploting low rank structure, several methods   circumvent this problem (cite spectral bundle, macedo's paper). In general, however, it is not entirely assured that the solution to the convexified problem is low-rank itself, and even less gauranteed for the intermediate iterates.

The  approach behind the second class of methods is to force low-rank parsimony of the intermediate and final iterates at the expense of a global optimality gaurantee. (cite burer monteiro, others) Our method falls in this category, and we can gaurantee only convergence to a global stationary point. However, several recent papers (boumal) suggest that with high probability, with $k$ large enough, that such local optima are of high quality, and often global optima. Thus, this can be seen as a tradeoff between the first and third category of methods--a small sacrifice in theoretical comfort for scalability, but over a wider class of nonconvex problems.

Specifically, problem \eqref{eq:main} is nonconvex in both the objective and constraint, and thus the convergence of alternating methods like ADMM on \eqref{eq:main} is not well understood. The main contribution of this paper is to show that ADMM on an equivalent reformulation of \eqref{eq:main} converges to a stationary point, and whose stationary solutions are of high quality in many practical applications.

\paragraph{This is for non-linearized ADMM}

The joint minimization of $X$ and $Z$ is now solution to the linear system
\begin{equation*}
\begin{array}{rcl}
\big(C - \mA^*(\nu) + S + \rho(Z-XY^T)\big)_\Omega &=& 0\\
U -S_\Omega Y + \rho(XY^T - Z)_\Omega Y + \rho(X-Y) &=& 0\\
\mA(Z) &=& b.
\end{array}
%\label{eq:z1z2OptCond}
\end{equation*}
where $\nu\in\reals^m$  is the dual variable for the local constraint $\mA(X) = b$.


Given $Y$, solving for $\nu$ reduces to solving
\[
G\nu = \mA(\mA^*(\nu)(YY^T + I)) = \rho(b-\mA(DY^T)) + \mA[(C+S)(I + YY^T)]
\]
where
\[
D =  \frac{1}{\rho}(S_\Omega Y -U) + Y , \quad
G_{ij} = \langle A_i, A_j(YY^T + I)\rangle .
\]
In the case where $\langle A_i,A_j\rangle = 0,\forall 1\le i\ne j\le m$, $G$ is a diagonal positive definite matrix then finding $G^{-1}$ is computationally simple.
Then
\[
X = BY + D, \quad \text{ and } \quad
Z_\Omega = \big(XY^T\big)_\Omega + B,
\]
where
\[
B = \big(-\frac{1}{\rho}(C-\mA^*(\nu) + S)\big)_\Omega.
\]
Note that the complexity of all inversions are $O(r^{3})$, and are particularly simple if $r = 1$. In that case, the complexity is dominated by the matrix multiplications. Also, for the cases without the linear constraint $\mA(Z) = b$, the solution for $(Z,X)$ is straightforward.





==> wasted/ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{An Example Article\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

